Can Demographic Factors Improve Text Classification? Revisiting Demographic Adaptation in the Age of Transformers

Demographic factors (e.g., gender or age) shape our language. Previous work showed that incorporating demographic factors can consistently improve performance for various NLP tasks with traditional NLP models. In this work, we investigate whether these previous findings still hold with state-of-the-art pretrained Transformer-based language models (PLMs). We use three common specialization methods proven effective for incorporating external knowledge into pretrained Transformers (e.g., domain-specific or geographic knowledge). We adapt the language representations for the demographic dimensions of gender and age, using continuous language modeling and dynamic multi-task learning for adaptation, where we couple language modeling objectives with the prediction of demographic classes. Our results, when employing a multilingual PLM, show substantial gains in task performance across four languages (English, German, French, and Danish), which is consistent with the results of previous work. However, controlling for confounding factors - primarily domain and language proficiency of Transformer-based PLMs - shows that downstream performance gains from our demographic adaptation do not actually stem from demographic knowledge. Our results indicate that demographic specialization of PLMs, while holding promise for positive societal impact, still represents an unsolved problem for (modern) NLP.

==> 06-reproducibility.tex <==
\vspace{-0.2em}
To ensure full reproducibility of our results and fuel further research on demographic adaptation in NLP, our resources are publicly available at:
\url{https://github.com/umanlp/SocioAdapt}.
\vspace{-0.3em}

==> 10-gender-tables.tex <==
\setlength{\tabcolsep}{2.3pt} %5.5
\begin{table*}[t]
\centering
%\resizebox{\textwidth}{!}{%
\footnotesize{
\begin{tabular}{llcccccgcccccg}
\toprule
                                 &                              & \multicolumn{6}{c}{\textbf{AC-SA}}                                                                                                      & \multicolumn{6}{c}{\textbf{AC-TD}}                                                                                                      \\ \cmidrule(lr){3-8}\cmidrule(lr){9-14}
       \textbf{Model}                          &                              & \textbf{US}          & \textbf{Denmark}     & \textbf{Germany}     & \textbf{France}      & \textbf{UK}          & \textbf{Avg.}        & \textbf{US}          & \textbf{Denmark}     & \textbf{Germany}     & \textbf{France}      & \textbf{UK}          & \textbf{Avg.}        \\\midrule
\multirow{6}{*}{\textit{\textbf{gender}}} & \textit{w/o specialization}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                 & mBERT                        & 62.6                 & 64.0                 & 59.5                 & 63.9                 & 61.9                 & 62.4                 & 58.1                 & 61.8                 & 57.9                 & 61.2                 & 63.1                 & 60.4                 \\\cmidrule{2-14}
                                 & \textit{with specialization} &                      &                      &                      &                      &                      &         \multicolumn{1}{c}{}              &                      &                      &                      &                      &                      &      \multicolumn{1}{c}{}                 \\
                                 & MLM                          & 63.3                 & \textbf{65.2}                 & 61.2                 & 64.6                 & 63.0                 & 63.4                 & \textbf{59.6}                 & 63.4                 & 60.1                 & 62.1                 & 65.3                 & 62.1                 \\
                                 & MTL-W (CLS)                  & \textbf{63.8}                 & 64.9                 & 60.1                 & 64.1                 & 63.4                 & 63.3                 & 59.2                 & 63.5                 & \textbf{60.3}                 & \textbf{63.1}                 & 64.9                 & \textbf{62.2}                 \\
                                 & MTL-W (CTX)                  & 62.2                 & 65.0                 & \textbf{62.9}                 & \textbf{65.0}                 & \textbf{63.5}                 & \textbf{63.7}                 & 58.8                 & \textbf{63.5}                 & 58.3                 & 62.9                 & \textbf{65.6}                 & 61.8                 \\
                                 \midrule
\multirow{6}{*}{\textit{\textbf{age}}}    & \textit{w/o specialization}  &                      &                      &                      &                      &                      &      \multicolumn{1}{c}{}                 &                      &                      &                      &                      &                      &        \multicolumn{1}{c}{}               \\
                                 & mBERT                        & 62.9                 & 57.2                 & 58.0                 & 55.7                 & 65.1                 & 59.8                 & 60.7                 & 64.5                 & 56.9                 & 56.6                 & 65.2                 & 60.8                 \\\cmidrule{2-14}
                                 & \textit{with specialization} &                      &                      &                      &                      &                      &        \multicolumn{1}{c}{}               &                      &                      &                      &                      &                      &        \multicolumn{1}{c}{}               \\
                                 & MLM                          & \textbf{63.6}                 & \textbf{65.5}                 & \textbf{61.1}                 & \textbf{56.8}                 & \textbf{65.4}                 & \textbf{62.5}                 & \textbf{61.9}                 & 65.1                 & \textbf{58.9}                 & \textbf{57.2}                 & \textbf{65.6}                 & \textbf{61.7}                 \\
                                 & MTL-W (CLS)                  & 60.7                 & 65.2                 & 56.4                 & 55.1                 & 65.3                 & 60.5                 & 61.5                 & \textbf{65.2}                 & 58.2                 & 55.5                 & 62.8                 & 60.6                 \\
                                 & MTL-W (CTX)                  & 59.7                 & 65.3                 & 56.6                 & 54.4                 & 64.0                 & 60.0                 & 61.2                 & 64.6                 & 57.4                 & 55.9                 & 62.8                 & 60.4     \\
                                 \bottomrule
\end{tabular}%
}
\caption{Intrinsic evaluation results for \textit{gender} and \textit{age} on Attribute Classification (AC-SA, AC-TD). We report the F1-score and compare the specialized models (MLM, MTL-W (CLS), MTL-W (CTX)) with vanilla mBERT.}
\label{tab:gender_age_intrinsic}
\vspace{-0.7em}
\end{table*}

% \setlength{\tabcolsep}{5.9pt}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% %\resizebox{\textwidth}{!}{%
% \scriptsize{
% \begin{tabular}{lcccccgcccccg}
% \toprule
%                     & \multicolumn{6}{c}{\textbf{AC-SA (\textit{gender})}}                                                                                & \multicolumn{6}{c}{\textbf{AC-TD (\textit{gender})}}                                                                   \\
% \textbf{Model}                    & \textbf{US} & \textbf{Denmark}     & \textbf{Germany}     & \textbf{France}      & \textbf{UK} & \textbf{Avg.} & \textbf{US} & \textbf{Denmark} & \textbf{Germany} & \textbf{France} & \textbf{UK} & \textbf{Avg.} \\ \cmidrule(lr){2-7}\cmidrule(lr){8-13}
%                     %\midrule
% \textit{w/o specialization}   & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    &  \multicolumn{1}{c}{}                      &                  &                  &                 &    & &   \multicolumn{1}{c}{}                  \\
% mBERT               & 62.60                  & 63.96                & 59.50                & 63.93                & 61.89     &     62.38         & 58.11                  & 61.84            & 57.94            & 61.20           & 63.14         &  60.45        \\
% \midrule
% \textit{with specialization} &                        &                      &                      &                      &                         &                      \multicolumn{1}{c}{}    &               &                  &                 &      & &      \multicolumn{1}{c}{}             \\
% MLM              & 63.28                  & 65.23                & 61.18                & 64.58                & 62.96        &    63.45       & \textbf{59.56}                  & 63.41            & 60.09            & 62.11           & 65.25        & 62.08          \\
% MTL-W (CLS)              & \textbf{63.84}                  & 64.86                & 60.08                & 64.08                & 63.42   &     63.26           & 59.15                  & 63.46            & \textbf{60.31}            & \textbf{63.06}           & 64.91        &     \textbf{62.18}     \\
% MTL-W (CTX)          & 62.19                  & \textbf{64.95}                & \textbf{62.86}                & \textbf{65.03}                & \textbf{63.54}  &            \textbf{63.71}     & 58.81                  & \textbf{63.48}            & 58.30            & 62.94           & \textbf{65.61}          & 61.83\\
% \bottomrule
% \end{tabular}%
% }
% \caption{Attribute classification results for \textit{gender} with F1 score.}
% \label{tab:gender_intrinsic}
% \end{table*}

==> 11-age-tables.tex <==
\setlength{\tabcolsep}{3pt} %4.7
\begin{table*}[t]
\centering
\footnotesize{
%\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccccccccccg}
\toprule
                                      &                              & \multicolumn{3}{c}{\textbf{US}}               & \multicolumn{3}{c}{\textbf{Denmark}}          & \multicolumn{3}{c}{\textbf{Germany}}          & \multicolumn{3}{c}{\textbf{France}}           & \multicolumn{3}{c}{\textbf{UK}}               &\multicolumn{1}{l}{} \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
                                       \textit{\textbf{gender}} &  \textbf{Model}                            & \textbf{F}    & \textbf{M}    & \textbf{X} \textbf{}   & \textbf{F}    & \textbf{M}    & \textbf{X}    & \textbf{F}    & \textbf{M}    & \textbf{X}    & \textbf{F}    & \textbf{M}    & \textbf{X}    & \textbf{F}    & \textbf{M}    & \textbf{X}    &  \textbf{Avg.}    \\ \cmidrule{1-17}
\multirow{6}{*}{\textbf{SA}} & \textit{w/o specialization}  &               &               &               &               &               &               &               &               &               &               &               &               &               &               &               & \multicolumn{1}{l}{}              \\
                                      & mBERT                        & 66.3          & 64.4          & 66.0          & 69.2          & 64.8          & 67.2          & 66.1          & 63.2          & 64.5          & 69.3          & 67.0          & 67.8          & 71.0          & 69.0          & 69.7          & 67.0          \\\cmidrule{2-17}
                                      & \textit{with specialization} &               &               &               &               &               &               &               &               &               &               &               &               &               &               &               &   \multicolumn{1}{l}{}            \\
                                      & MLM                          & 67.3          & 66.2          & 66.9          & 69.5          & \textbf{65.8} & 67.8          & \textbf{67.7} & \textbf{65.3} & 66.1          & 69.9          & 67.1          & 68.4          & 72.0          & 70.4          & 71.0          & 68.1          \\
                                      & MTL-W (CLS)                  & 67.2          & 66.3          & 67.0          & \textbf{69.9} & 65.7          & 67.7          & 66.7          & 64.0          & 65.7          & \textbf{70.6} & 67.3          & 68.4          & 72.9          & 70.9          & 71.7          & 68.1          \\
                                      & MTL-W (CTX)                  & \textbf{68.0} & \textbf{66.4} & \textbf{67.3} & 69.1          & 65.6          & \textbf{68.0} & 66.8          & 64.3          & \textbf{66.8} & 70.1          & \textbf{67.5} & \textbf{68.8} & \textbf{73.0} & \textbf{71.0} & \textbf{71.9} & \textbf{68.3} \\ \cmidrule{1-17}
\multirow{6}{*}{\textbf{TD}} & \textit{w/o specialization}  &               &               &               &               &               &               &               &               &               &               &               &               &               &               &               & \multicolumn{1}{l}{}              \\
                                      & mBERT                        & 71.2          & 68.4          & 70.2          & 59.3          & 58.3          & 59.0          & 67.8          & 65.6          & 65.8          & 44.6          & 42.4          & 43.1          & 70.4          & 67.9          & 68.9          & 61.5          \\\cmidrule{2-17}
                                      & \textit{with specialization} &               &               &               &               &               &               &               &               &               &               &               &               &               &               &               & \multicolumn{1}{l}{}              \\
                                      & MLM                          & 72.1          & 69.4          & 70.3          & 59.7          & 58.8          & \textbf{59.4} & \textbf{68.6} & 67.0          & \textbf{67.1} & 45.8          & 43.3          & 44.3          & 70.6          & 67.9          & 69.8          & 62.3          \\
                                      & MTL-W (CLS)                  & 72.3          & 69.2          & 70.4          & 59.7          & 57.8          & 59.1          & 67.6          & 65.7          & 66.4          & \textbf{46.0} & 43.4          & 44.2          & 70.6          & 68.2          & 69.8          & 62.0          \\
                                      & MTL-W (CTX)                  & \textbf{72.8} & \textbf{69.5} & \textbf{70.5} & \textbf{59.9} & \textbf{58.9} & 59.0          & 68.3          & \textbf{67.0} & 66.7          & 45.5          & \textbf{43.9} & \textbf{44.4} & \textbf{70.8} & \textbf{68.2} & \textbf{69.9} & \textbf{62.4}\\
                                      \bottomrule
\end{tabular}%
}
\caption{Results of the extrinsic evaluation on \textit{gender} data for gender-specialized and non-specilized models for Sentiment Analysis (SA) and Topic Detection (TD). We report the F1-score.}
\vspace{-0.3em}
\label{tab:gender_task}
\end{table*}

\setlength{\tabcolsep}{3.4pt} %5pt
\begin{table*}[t]
\centering
%\resizebox{\textwidth}{!}{%
\footnotesize{
\begin{tabular}{llcccccccccccccccg}
\toprule
                                   &                              & \multicolumn{3}{c}{\textbf{US}}                                    & \multicolumn{3}{c}{\textbf{Denmark}}                               & \multicolumn{3}{c}{\textbf{Germany}}                               & \multicolumn{3}{c}{\textbf{France}}                                & \multicolumn{3}{c}{\textbf{UK}}                        &   \multicolumn{1}{l}{}      \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
                                   \textit{\textbf{age}} &       \textbf{Model}                       & \textbf{<35}           & \textbf{>45}           & \textbf{X}           & \textbf{<35}           & \textbf{>45}           & \textbf{X}           & \textbf{<35}           & \textbf{>45}           & \textbf{X}           & \textbf{<35}           & \textbf{>45}           & \textbf{X}           & \textbf{<35}           & \textbf{>45}           & \textbf{X}           & \textbf{Avg.}           \\\cmidrule{1-17}
\multirow{6}{*}{\textbf{SA}} & \textit{w/o specialization}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                   & mBERT                        & 57.7                 & 57.9                 & 57.8                 & 62.7                 & 62.7                 & 62.9                 & 52.6                 & 55.0                 & 55.0                 & 59.6                 & 57.4                 & 61.5                 & 63.8                 & 63.9                 & 63.7                 & 59.6                 \\\cmidrule{2-17}
                                   & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &        \multicolumn{1}{l}{}              \\
                                   & MLM                          & 59.4                 & 57.8                 & \textbf{58.2}        & 63.3                 & 62.1                 & 63.0                 & 53.6                 & 55.5                 & 56.7                 & 59.9                 & 59.5                 & 61.6                 & 62.8                 & 62.0                 & 63.0                 & 59.9                 \\
                                   & MTL-W (CLS)                  & 59.3                 & 57.9                 & 58.0                 & 63.1                 & 62.9                 & 63.0                 & \textbf{53.8}        & 55.3                 & 55.5                 & 60.4                 & \textbf{60.3}        & \textbf{62.8}        & 63.8                 & 64.9                 & 64.9                 & 60.4                 \\
                                   & MTL-W (CTX)                  & \textbf{59.9}        & \textbf{58.6}        & 57.8                 & \textbf{64.2}        & \textbf{63.3}        & \textbf{63.2}        & 53.0                 & \textbf{56.5}        & \textbf{56.7}        & \textbf{60.9}        & 59.8                 & 59.7                 & \textbf{64.6}        & \textbf{65.2}        & \textbf{65.1}        & \textbf{60.6}        \\\cmidrule{1-17}
\multirow{6}{*}{\textbf{TD}} & \textit{w/o specialization}  &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &       \multicolumn{1}{l}{}               \\
                                   & mBERT                        & 68.0                 & 64.3                 & 64.3                 & 56.1                 & 52.2                 & 53.4                 & 60.1                 & 55.3                 & 57.1                 & 52.0                 & 47.1                 & 49.0                 & 64.7                 & 67.1                 & 66.3                 & 58.5                 \\\cmidrule{2-17}
                                   & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &       \multicolumn{1}{l}{}               \\
                                   & MLM                          & 69.0                 & 64.2                 & 65.2                 & \textbf{57.1}        & 52.6                 & 54.1                 & \textbf{61.5}        & 56.5                 & 58.7                 & \textbf{52.5}        & 47.2                 & 50.3                 & 65.1                 & 67.3                 & 67.3                 & 59.2                 \\
                                   & MTL-W (CLS)                  & \textbf{69.8}        & 64.4                 & \textbf{65.8}        & 56.9                 & \textbf{53.3}        & \textbf{54.5}        & 60.8                 & \textbf{57.6}        & \textbf{59.3}        & 51.1                 & 47.3                 & 50.3                 & 66.0                 & \textbf{68.1}        & 66.5                 & \textbf{59.4}        \\
                                   & MTL-W (CTX)                  & 69.2                 & \textbf{65.4}        & 64.9                 & 56.2                 & 53.2                 & 54.3                 & 59.3                 & 56.5                 & 59.3                 & 50.2                 & \textbf{48.0}        & \textbf{50.8}        & \textbf{66.4}        & 67.3                 & \textbf{67.6}        & 59.2\\ \bottomrule                
\end{tabular}%
}
\caption{Results of the extrinsic evaluation on \textit{age} data for age-specialized and non-specialized models for Sentiment Analysis (SA) and Topic Detection (TD). We report the F1-score.}
\vspace{-0.3em}
\label{tab:age_task}
\end{table*}
% \setlength{\tabcolsep}{3.9pt}
% \begin{table*}[t]
% \centering
% %\resizebox{\textwidth}{!}{%
% \scriptsize{
% \begin{tabular}{clccccccccccccccc}
% \toprule
% \multicolumn{1}{l}{}                &            & \multicolumn{3}{c}{\textbf{US}} & \multicolumn{3}{c}{\textbf{Denmark}} & \multicolumn{3}{c}{\textbf{Germany}} & \multicolumn{3}{c}{\textbf{France}} & \multicolumn{3}{c}{\textbf{UK}} \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
% %\midrule
% %\multicolumn{1}{l}{}                &            & F         & M         & X         & F       & M       & X       & F       & M       & X       & F       & M       & X      & F          & M         & X         \\
% \multicolumn{1}{l}{}                &  \textbf{Model}           & \textbf{F} & \textbf{M} & \textbf{X} & \textbf{F} & \textbf{M} & \textbf{X} & \textbf{F} & \textbf{M} & \textbf{X} & \textbf{F} & \textbf{M} & \textbf{X} & \textbf{F} & \textbf{M} & \textbf{X} \\
% \midrule
% \multirow{6}{*}{\textbf{SA (\textit{gender})}} & \textit{w/o specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     & \\
% & mBERT     &    66.30     &    64.37     &    65.98     &   69.18      &    64.80     &  67.21      &     66.12   &  63.18       &    64.45     &    69.30     &     66.99    &     67.82    &   71.04     &  69.04   & 69.74\\ \cmidrule{2-17}
% & \textit{with specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     & \\
%                                     & MLM    & 67.32     & 66.20      & 66.89     & 69.48   & \textbf{65.77}   & 67.77   & \textbf{67.71}   & \textbf{65.32}   & 66.13   & 69.86   & 67.09   & 68.36  & 71.99      & 70.61     & 71.04     \\
%                                     & MTL-W (CLS)     & 67.19     & 66.31     & 66.98     & \textbf{69.89}   & 65.65   & 67.65   & 66.74   & 64.04   & 65.74   & \textbf{70.57}   & 67.31   & 68.40   & 72.87      & 70.90      & 71.65     \\
%                                     & MTL-W (CTX) & \textbf{67.98}     & \textbf{66.44}     & \textbf{67.28}     & 69.11   & 65.59   & \textbf{67.95}   & 66.82   & 64.32   & \textbf{66.78}   & 70.14   & \textbf{67.46}   & \textbf{68.81}  &      \textbf{72.95}      &     \textbf{70.99}      & \textbf{71.94}     \\
%                                     \midrule
% \multirow{6}{*}{\textbf{TD (\textit{gender})}} & \textit{w/o specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     & \\
% & mBERT     &   71.15      &    68.44     &    70.20     &   59.28      &    58.27     &   58.99     &  67.77      &  65.63       &   65.80      &   44.55      &    42.37     &   43.05      &   70.41     &  67.89   & 68.86\\ \cmidrule{2-17}
% & \textit{with specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     & \\
%                                     & MLM     & 72.11     & 69.37     & 70.27     & 59.66   & 58.76   & \textbf{59.35}   &   \textbf{68.56}     &    66.97     &     \textbf{67.13}    &  45.78       &   43.34      &  44.25      & 70.60      & 67.93     & 69.80     \\
%                                     & MTL-W (CLS)     & 72.34     & 69.22     & 70.44     & 59.72   & 57.78   & 59.05   &   67.61      &   65.65      &   66.40      &  \textbf{46.04}       &  43.38       &   44.17     & 70.63      & 68.22     & 69.78     \\
%                                     & MTL-W (CTX) & \textbf{72.83}     & \textbf{69.50}      & \textbf{70.53}     & \textbf{59.86}   & \textbf{58.88}   & 58.98   &    68.34     &   \textbf{66.98}      &   66.74      &    45.46     &   \textbf{43.85}      &  \textbf{44.38}      & \textbf{70.78}      & \textbf{68.24}     & \textbf{69.92} \\
%                                     \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation results on \textit{gender} data on two tasks: sentiment analysis (SA) and topic detection (TD) with F1 score.}
% \label{tab:gender_task_old}
% \end{table*}

% \setlength{\tabcolsep}{5.9pt}
% \begin{table*}[t!]
% \centering
% %\resizebox{\textwidth}{!}{%
% \scriptsize{
% \begin{tabular}{lcccccgcccccg}
% \toprule
%                     & \multicolumn{6}{c}{\textbf{AC-SA (\textit{age})}}                                                          & \multicolumn{6}{c}{\textbf{AC-TD (\textit{age})}}                                                          \\
%     \textbf{Model}                 & \textbf{US} & \textbf{Denmark} & \textbf{Germany} & \textbf{France} & \textbf{UK} & \textbf{Avg.} & \textbf{US} & \textbf{Denmark} & \textbf{Germany} & \textbf{France} & \textbf{UK} & \textbf{Avg.} \\\cmidrule(lr){2-7}\cmidrule(lr){8-13}
% \textit{w/o specialization}   &                        &                  &                  &                 &             &         \multicolumn{1}{c}{}                 &                  &                  &                 &         &&   \multicolumn{1}{c}{}   \\
% mBERT               & 62.93                  & 57.16            & 58.03            & 55.72           & 65.13       &  59.79 & 60.73                  & 64.51            & 56.92            & 56.57           & 65.19    &  60.78 \\
% \midrule
% \textit{with specialization} &                        &                  &                  &                 &             &      \multicolumn{1}{c}{}                  &                   &                  &                 &          &&  \multicolumn{1}{c}{}   \\
% MLM              & \textbf{63.63}                  & \textbf{65.46}            & \textbf{61.12}            & \textbf{56.84}           & \textbf{65.38}       & \textbf{62.49} & \textbf{61.86}                  & 65.08            & \textbf{58.92}            &  \textbf{57.15}           & \textbf{65.63}       & \textbf{61.73}\\
% MTL-W (CLS)             & 60.73                  & 65.21            & 56.39            & 55.06           & 65.28     & 60.53 & 61.54                  & \textbf{65.24}            & 58.16            & 55.50           & 62.80     & 60.65 \\
% MTL-W (CTX)          & 59.71                  & 65.30            & 56.55            & 54.40            & 63.96   &  59.98  & 61.21                  & 64.63            & 57.39            & 55.88           & 62.76     & 60.37\\
% \bottomrule
% \end{tabular}%
% }
% \caption{Attribute classification results for \textit{age} with F1 score.}
% \label{tab:age_intrinsic}
% \end{table*}

% \setlength{\tabcolsep}{4.2pt}
% \begin{table*}[t!]
% \centering
% %\resizebox{\textwidth}{!}{%
% \scriptsize{
% \begin{tabular}{llccccccccccccccc}
% \toprule
%                                  &                 & \multicolumn{3}{c}{\textbf{US}} & \multicolumn{3}{c}{\textbf{Denmark}} & \multicolumn{3}{c}{\textbf{Germany}} & \multicolumn{3}{c}{\textbf{France}}  & \multicolumn{3}{c}{\textbf{UK}} \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
%                                  &      \textbf{Model}            & \textbf{0}   & \textbf{2}   & \textbf{X}   & \textbf{0} & \textbf{2} & \textbf{X} & \textbf{0} & \textbf{2} & \textbf{X} & \textbf{0} & \textbf{2} & \textbf{X} & \textbf{0}    & \textbf{2}   & \textbf{X}  \\
%                                  \midrule
% \multirow{6}{*}{\textbf{SA (\textit{age})}} & \textit{w/o specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     & \\
% & mBERT     &    57.65     &   57.87      &   57.79      &    62.72     &    62.65     &    62.93    &  52.63      &  54.97       &   55.03      &    59.56     &     57.39    &    61.50     &    63.79    & 63.90    & 63.69 \\ \cmidrule{2-17}
% & \textit{with specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     & \\
%                                  & MLM          & 59.35        & 57.80        & \textbf{58.24}        & 63.30       & 62.08      & 62.96      & 53.60       & 55.51      & 56.67      & 59.85      & 59.46      & 61.62      & 62.84         & 61.96        & 63.00      \\
%                                  & MTL-W (CLS)          & 59.32        & 57.91        & 58.01        & 63.14      & 62.93      & 63.01      & \textbf{53.80}       & 55.33      & 55.54      & 60.40       & \textbf{60.28}      & \textbf{62.78}      & 63.81         & 64.86        & 64.92    \\
%                                  & MTL-W (CTX)      & \textbf{59.88}        & \textbf{58.58}        & 57.77        & \textbf{64.18}      & \textbf{63.34}      & \textbf{63.16}      & 52.97      & \textbf{56.45}      & \textbf{56.74}      & \textbf{60.87}      & 59.81      & 59.66      & \textbf{64.60}         & \textbf{65.22}        & \textbf{65.06}   \\
%                                  \midrule
% \multirow{6}{*}{\textbf{TD (\textit{age})}} &\textit{w/o specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &     &  \\
% & mBERT     &    67.96     &    64.30     &    64.33     &      56.13   &    52.18     &     53.44   &     60.08   &     55.30   &    57.07     &    52.02     &    47.05     &    48.95     &   64.69     &   67.09  &  66.27\\ \cmidrule{2-17}
% & \textit{with specialization}     &         &         &         &         &         &        &        &         &         &         &         &         &        &   &  \\
%                                  & MLM          & 68.97        & 64.17        & 65.21        & \textbf{57.12}      & 52.64      & 54.10       & \textbf{61.49}      & 56.46      & 58.67      & \textbf{52.52}      & 47.22      & 50.32      & 65.10         & 67.26        & 67.31    \\
%                                  & MTL-W (CLS)         & \textbf{69.79}        & 64.37        & \textbf{65.80}        & 56.93      & \textbf{53.33}      & \textbf{54.54}      & 60.79      & \textbf{57.64}      & \textbf{59.31}      & 51.11      & 47.28      & 50.29      & 65.96         & \textbf{68.05}        & 66.48 \\
%                                  & MTL-W (CTX)      & 69.24        & \textbf{65.37}        & 64.93        & 56.18      & 53.18      & 54.29      & 59.28      & 56.48      & 59.30      & 50.19      & \textbf{48.02}      & \textbf{50.78}      & \textbf{66.35}         & 67.30        & \textbf{67.62} \\
%                                  \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation results on \textit{age} data on two tasks: sentiment analysis (SA) and topic detection (TD) with F1 score.}
% \label{tab:age_task_old}
% \end{table*}

==> 12-mono-multi-tables.tex <==
\setlength{\tabcolsep}{2.3pt}
\begin{table*}[t]
\centering
%\resizebox{\textwidth}{!}{%
\footnotesize{
\begin{tabular}{llcccccccccccccccc}
\toprule
                                  &                              & \multicolumn{8}{c}{\textit{\textbf{gender}}}                                                                                                                                                   & \multicolumn{8}{c}{\textit{\textbf{age}}}                                                                                                                                                      \\
                                  \cmidrule(lr){3-10}\cmidrule(lr){11-18}
                                  &                              & \multicolumn{1}{c}{\textbf{AC-SA}}       & \multicolumn{1}{c}{\textbf{AC-TD}}       & \multicolumn{3}{c}{\textbf{SA}}                                    & \multicolumn{3}{c}{\textbf{TD}}                                    & \multicolumn{1}{c}{\textbf{AC-SA}}       & \multicolumn{1}{c}{\textbf{AC-TD}}       & \multicolumn{3}{c}{\textbf{SA}}                                    & \multicolumn{3}{c}{\textbf{TD}}                                    \\
                                  &   &     \multicolumn{1}{c}{$\Delta$}                 &       \multicolumn{1}{c}{$\Delta$}               &         \multicolumn{3}{c}{$\Delta$}                  &                    \multicolumn{3}{c}{$\Delta$}           &   \multicolumn{1}{c}{$\Delta$}                 &       \multicolumn{1}{c}{$\Delta$}               &         \multicolumn{3}{c}{$\Delta$}                  &                    \multicolumn{3}{c}{$\Delta$}  \\ \cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-11}\cmidrule(lr){12-12}\cmidrule(lr){13-15}\cmidrule(lr){16-18}
                                  & \textbf{Model}               & \textbf{}            & \textbf{}            & \multicolumn{1}{c}{\textbf{F}}           & \multicolumn{1}{c}{\textbf{M}}           & \multicolumn{1}{c}{\textbf{X}}           & \multicolumn{1}{c}{\textbf{F}}           & \multicolumn{1}{c}{\textbf{M}}           & \multicolumn{1}{c}{\textbf{X}}          & \textbf{}            & \textbf{}            & \multicolumn{1}{c}{\textbf{<35}}            & \multicolumn{1}{c}{\textbf{>45}}           & \multicolumn{1}{c}{\textbf{X}}           & \multicolumn{1}{c}{\textbf{<35}}            & \multicolumn{1}{c}{\textbf{>45}}            & \multicolumn{1}{c}{\textbf{X}}           \\ \midrule
\multirow{5}{*}{\textbf{US}} & \textit{w/o specialization}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\                    
                                                     & BERT                         & 1.7                  & 0.5                  & 2.3                  & 2.6                  & 1.1                  & 1.4                  & 1.3                  & 0.8                  & 2.3                  & 2.3                  & 2.8                  & 0.8                  & -0.6                 & 0.8                  & 0.6                  & 2.8                  \\\cmidrule{2-18}
                                                     & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                                     & MLM                          & 1.3                  & -0.9                 & 1.1                  & 1.4                  & 0.9                  & 1.0                  & 0.7                  & 1.0                  & 1.6                  & 2.3                  & 0.5                  & 1.7                  & 2.1                  & 2.2                  & 1.5                  & 1.5                  \\
                                                     & MTL-W (CTX)                  & 2.5                  & 0.6                  & 0.9                  & 1.1                  & 0.6                  & 0.4                  & 0.4                  & 1.1                  & 6.0                  & 2.0                  & 1.2                  & 0.1                  & 1.7                  & 0.2                  & 0.3                  & 1.8                  \\
                                                     \midrule
\multirow{5}{*}{\textbf{Denmark}}                    & \textit{w/o specialization}  &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                                     & BERT                         & 2.1                  & 2.0                  & 3.1                  & 3.1                  & 3.2                  & 1.4                  & 1.5                  & 0.9                  & 10.6                 & 0.8                  & 4.5                  & 3.6                  & 3.1                  & 2.3                  & 2.2                  & 2.9                  \\\cmidrule{2-18}
                                                     & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                                     & MLM                          & 0.8                  & 0.7                  & 3.1                  & 2.5                  & 2.5                  & 1.0                  & 1.9                  & 1.3                  & 2.0                  & 2.3                  & 4.4                  & 5.3                  & 4.6                  & 2.1                  & 2.7                  & 3.5                  \\
                                                     & MTL-W (CTX)                  & 1.1                  & 0.6                  & 3.3                  & 2.8                  & 2.6                  & 1.3                  & 1.3                  & 1.8                  & 2.5                  & 2.0                  & 3.4                  & 2.8                  & 4.0                  & 2.8                  & 2.2                  & 2.5                  \\ \midrule
\multirow{5}{*}{\textbf{Germany}}                    & \textit{w/o specialization}  &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                                     & BERT                         & 0.3                  & 1.0                  & 0.4                  & 0.5                  & -0.2                 & 0.2                  & 0.5                  & 2.0                  & -0.1                 & 2.7                  & 1.0                  & 2.9                  & 2.1                  & 1.5                  & 2.1                  & 1.3                  \\\cmidrule{2-18}
                                                     & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                                     & MLM                          & 0.8                  & -0.4                 & 0.4                  & 0.5                  & -0.8                 & 0.0                  & -0.3                 & 0.6                  & -3.0                 & 3.1                  & 4.5                  & 2.7                  & 1.4                  & 0.7                  & 1.1                  & 1.2                  \\
                                                     & MTL-W (CTX)                  & -2.0                 & 2.0                  & 1.1                  & 1.3                  & -0.7                 & 0.2                  & -0.2                 & 1.1                  & 0.7                  & 3.3                  & 4.9                  & 1.6                  & -2.7                 & 4.2                  & 1.8                  & -0.1                 \\ \midrule
\multirow{5}{*}{\textbf{France}}  & \textit{w/o specialization}  &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      & \\
\multicolumn{1}{l}{}                                 & BERT                         & 0.1                  & 1.9                  & 1.2                  & 0.3                  & 0.8                  & 1.4                  & 2.1                  & 2.0                  & 0.2                  & 0.5                  & 0.2                  & 0.1                  & -1.2                 & -0.1                 & 2.1                  & 0.7                  \\\cmidrule{2-18}
\multicolumn{1}{l}{}                                 & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
\multicolumn{1}{l}{}                                 & MLM                          & 0.4                  & 1.1                  & 1.2                  & 0.6                  & -0.8                 & 0.4                  & 0.9                  & 1.3                  & -0.9                 & -0.2                 & 0.8                  & -0.1                 & 0.0                  & 1.3                  & 1.3                  & -0.1                 \\
\multicolumn{1}{l}{}                                 & MTL-W (CTX)                  & -0.7                 & 0.0                  & 1.6                  & 0.8                  & 0.6                  & 1.4                  & 0.5                  & 1.2                  & 1.4                  & 0.8                  & -0.7                 & 0.9                  & 1.8                  & 4.4                  & 3.4                  & -0.5                 \\ \midrule
\multirow{5}{*}{\textbf{UK}}      & \textit{w/o specialization}  &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
\multicolumn{1}{l}{}                                 & BERT                         & 1.3                  & 1.9                  & 2.4                  & 2.0                  & 2.5                  & 0.7                  & 1.2                  & 1.3                  & 0.6                  & 0.6                  & 1.4                  & 2.4                  & 1.8                  & 3.4                  & 1.0                  & 1.7                  \\\cmidrule{2-18}
\multicolumn{1}{l}{}                                 & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
\multicolumn{1}{l}{}                                 & MLM                          & 0.7                  & -0.5                 & 1.9                  & 0.6                  & 1.5                  & 0.6                  & 1.4                  & 0.2                  & 1.5                  & 0.4                  & 5.4                  & 5.3                  & 3.9                  & 3.7                  & 2.9                  & 2.7                  \\
\multicolumn{1}{l}{}                                 & MTL-W (CTX)                  & -0.2                 & -0.8                 & 0.8                  & 1.0                  & 0.2                  & 0.6                  & 0.9                  & 0.4                  & 2.8                  & 2.5                  & 3.0                  & 1.3                  & 2.1                  & 1.9                  & 2.3                  & 1.6                   \\
\bottomrule
\end{tabular}%
}
\caption{Results of the monolingual PLMs (BERT, germanBERT, danishBERT, frenchBERT) on Sentiment Analysis (SA), Topic Detection (TD), and Attribute Classification (AC-SA, AC-TD) with and without intermediate specialization for \emph{gender} and \emph{age} on the country-specific specialization portions of Trustpilot. We report the deltas in F1-score compared to the original results of the multilingual PLM (mBERT).} %The bracket indicates the negative value.}
\vspace{-0.3em}
\label{tab:mono-multi_compare}
\end{table*}

% \begin{table*}[t]
% \centering
% %\resizebox{\textwidth}{!}{%
% \scriptsize{
% \begin{tabular}{llcccccccccccccccc}
% \toprule
%                                   &                              & \multicolumn{8}{c}{\textbf{Gender}}                                                                                                                                                   & \multicolumn{8}{c}{\textbf{Age}}                                                                                                                                                      \\
%                                   \cmidrule(lr){3-10}\cmidrule(lr){11-18}
%                                   &                              & \textbf{AC-SA}       & \textbf{AC-TD}       & \multicolumn{3}{c}{\textbf{SA}}                                    & \multicolumn{3}{c}{\textbf{TD}}                                    & \textbf{AC-SA}       & \textbf{AC-TD}       & \multicolumn{3}{c}{\textbf{SA}}                                    & \multicolumn{3}{c}{\textbf{TD}}                                    \\
%                                   &   &     $\Delta$                 &       $\Delta$               &         \multicolumn{3}{c}{$\Delta$}                  &                    \multicolumn{3}{c}{$\Delta$}           &   $\Delta$                 &       $\Delta$               &         \multicolumn{3}{c}{$\Delta$}                  &                    \multicolumn{3}{c}{$\Delta$}  \\ \cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-11}\cmidrule(lr){12-12}\cmidrule(lr){13-15}\cmidrule(lr){16-18}
%                                   & \textbf{Model}               & \textbf{}            & \textbf{}            & \textbf{F}           & \textbf{M}           & \textbf{X}           & \textbf{F}           & \textbf{M}           & \textbf{X}           & \textbf{}            & \textbf{}            & \textbf{<35}           & \textbf{>45}           & \textbf{X}           & \textbf{<35}           & \textbf{>45}           & \textbf{X}           \\ \midrule
% \multirow{6}{*}{\textbf{Denmark}} & \textit{w/o specialization}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
%                                   & BERT                         & 2.1                  & 2.0                  & 3.1                  & 3.1                  & 3.2                  & 1.4                  & 1.5                  & 0.9                  & 10.6                 & 0.8                  & 4.5                  & 3.6                  & 3.1                  & 2.3                  & 2.2                  & 2.9                  \\ \cmidrule{2-18}
%                                   & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
%                                   & MLM                          & 0.8                  & 0.7                  & 3.1                  & 2.5                  & 2.5                  & 1.0                  & 1.9                  & 1.3                  & 2.0                  & 2.3                  & 4.4                  & 5.3                  & 4.6                  & 2.1                  & 2.7                  & 3.5                  \\
%                                   %& MTL-W (CLS)                  & 1.3                  & 0.6                  & 2.7                  & 3.0                  & 3.0                  & 1.6                  & 2.7                  & 0.9                  & 2.2                  & 1.6                  & 4.3                  & 3.3                  & 4.1                  & 1.7                  & 1.6                  & 2.0                  \\
%                                   & MTL-W (CTX)                  & 1.1                  & 0.6                  & 3.3                  & 2.8                  & 2.6                  & 1.3                  & 1.3                  & 1.8                  & 2.5                  & 2.0                  & 3.4                  & 2.8                  & 4.0                  & 2.8                  & 2.2                  & 2.5                  \\ \midrule
% \multirow{6}{*}{\textbf{Germany}} & \textit{w/o specialization}  &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
%                                   & BERT                         & 0.3                  & 1.0                  & 0.4                  & 0.5                  & -0.2                 & 0.2                  & 0.5                  & 2.0                  & -0.1                 & 2.7                  & 1.0                  & 2.9                  & 2.1                  & 1.5                  & 2.1                  & 1.3                  \\ \cmidrule{2-18}
%                                   & \textit{with specialization} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
%                                   & MLM                          & 0.8                  & -0.4                 & 0.4                  & 0.5                  & -0.8                 & 0.0                  & -0.3                 & 0.6                  & -3.0                 & 3.1                  & 4.5                  & 2.7                  & 1.4                  & 0.7                  & 1.1                  & 1.2                  \\
%                                   %& MTL-W (CLS)                  & 1.0                  & -1.3                 & 2.0                  & 0.4                  & 0.4                  & 1.3                  & 0.8                  & 1.3                  & 1.8                  & 3.2                  & 2.5                  & 1.9                  & 0.3                  & 2.7                  & 0.3                  & -0.2                 \\
%                                   & MTL-W (CTX)                  & -2.0                 & 2.0                  & 1.1                  & 1.3                  & -0.7                 & 0.2                  & -0.2                 & 1.1                  & 0.7                  & 3.3                  & 4.9                  & 1.6                  & -2.7                 & 4.2                  & 1.8                  & -0.1   \\
%                                   \bottomrule
% \end{tabular}%
% }
% \caption{Downstream task performance gains from the monolingual PLM (germanBERT, danishBERT) compared to multilingual PLM (mBERT) on non-specialized and specialized variants for two countries (Denmark, Germany) on two sociodemographic factors (age, gender).} %The bracket indicates the negative value.}
% \label{tab:mono-multi_compare}
% \end{table*}

% \setlength{\tabcolsep}{9.2pt}
% \begin{table*}[t]
% \centering
% %\resizebox{\textwidth}{!}{%
% \scriptsize{
% \begin{tabular}{rcccccccc}
% \toprule
% \multicolumn{1}{c}{}         & \multicolumn{4}{c}{\textbf{Gender-SA}}                                      & \multicolumn{4}{c}{\textbf{Gender-TD}}                                      \\
% \multicolumn{1}{c}{}         & \multicolumn{2}{c}{\textbf{monoBERT}} & \multicolumn{2}{c}{\textbf{mBERT}}  & \multicolumn{2}{c}{\textbf{monoBERT}} & \multicolumn{2}{c}{\textbf{mBERT}}  \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
% \textbf{Model}         & \textbf{Denmark}  & \textbf{Germany}  & \textbf{Denmark} & \textbf{Germany} & \textbf{Denmark}  & \textbf{Germany}  & \textbf{Denmark} & \textbf{Germany} \\
% \cmidrule(lr){2-5}\cmidrule(lr){6-9}
% \textit{No specialization}   &                   &                   &                  &                  &                   &                   &                  &                  \\
% monoBERT / mBERT                         & 66.09             & 59.79             & 63.96            & 59.50            & 63.79             & 58.91             & 61.84            & 57.94            \\
% \midrule
% \textit{With specialization} &                   &                   &                  &                  &                   &                   &                  &                  \\
% MLM                          & 66.03             & 61.98             & 65.23            & 61.18            & 64.15             & 59.73             & 63.41            & 60.09            \\
% MTL-W (CLS)                        &                   & 61.05             & 64.86            & 60.08            &                   & 58.52             & 63.46            & 60.31            \\
% MTL-W (CTX)                    &                   & 60.87             & 64.95            & 60.86            &                   & 60.26             & 63.48            & 58.30           \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Intrinsic classification results for gender with F1 score compared with monolingual and multilingual BERT model.}
% \label{tab:mono-multi-intrinsic}
% \end{table*}

==> 13-domain-tables.tex <==
% \setlength{\tabcolsep}{7.6pt}
% \begin{table*}[t]
% \centering
% %\resizebox{\textwidth}{!}{%
% \footnotesize{
% \begin{tabular}{clcccccccccccc}
% \toprule
% \multicolumn{1}{l}{}         &                & \multicolumn{6}{c}{\textit{\textbf{gender}}}                                         & \multicolumn{6}{c}{\textit{\textbf{age}}}                                                                                                  \\ \cmidrule(lr){3-8}\cmidrule(lr){9-14}
% \multicolumn{1}{l}{}         &                & \multicolumn{3}{c}{\textbf{SA}}      & \multicolumn{3}{c}{\textbf{TD}}      & \multicolumn{3}{c}{\textbf{SA}}                                 & \multicolumn{3}{c}{\textbf{TD}}                                 \\
% & & \multicolumn{3}{c}{$\Delta$}                  &                    \multicolumn{3}{c}{$\Delta$} & \multicolumn{3}{c}{$\Delta$}                  &                    \multicolumn{3}{c}{$\Delta$} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14} 
% \multicolumn{1}{l}{}         & \textbf{Model} & \textbf{F} & \textbf{M} & \textbf{X} & \textbf{F} & \textbf{M} & \textbf{X} & \textbf{\textless{}35} & \textbf{\textgreater{}45} & \textbf{X} & \textbf{\textless{}35} & \textbf{\textgreater{}45} & \textbf{X} \\ \midrule
% \multirow{2}{*}{\textbf{US}} & MLM            & -0.1       & -0.3       & -0.9       & -0.4       & -0.2       & -0.1       & -0.6                   & 0.0                       & -0.8       & -0.1                   & 0.0                       & -0.3       \\
%                              %& MTL-W (CLS)    & -0.6       & -0.6       & -1.1       & -0.3       & -1.0       & -0.3       & -0.2                   & -1.1                      & -0.5       & -0.3                   & -0.3                      & -0.7       \\
%                              & MTL-W (CTX)    & -0.3       & -0.4       & -1.5       & -0.8       & -0.3       & -0.4       & -0.3                   & -0.9                      & -0.5       & -0.1                   & 0.1                       & -0.7       \\ \midrule
% \multirow{2}{*}{\textbf{UK}} & MLM            & -0.6       & 0.0        & -0.8       & -0.1       & 0.0        & -0.3       & -2.0                   & -0.5                      & -0.5       & -1.0                   & -1.4                      & -1.1       \\
%                              %& MTL-W (CLS)    & -0.2       & -1.1       & -0.5       & -0.3       & -0.3       & -0.7       & -1.7                   & 0.2                       & -0.8       & 0.0                    & -0.2                      & -0.8       \\
%                              & MTL-W (CTX)    & -0.3       & -0.9       & -0.5       & -0.1       & 0.1        & -0.7       & -1.0                   & -0.5                      & -0.9       & -0.3                   & -0.8                      & 0.0     \\
%                              \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation results on Trustpilot for Sentiment Analysis (SA) and Topic Detection (TD) when running the intermediate specialization on out-of-domain data (RtGender~\citep{voigt-etal-2018-rtgender} for \textit{gender} and BAC~\citep{schler2006effects} for \textit{age}). We report the delta in F1-score in comparison to the specialization on in-domain data (Trustpilot).} 
% \label{tab:domain}
% \end{table*}
